Uncertainty-Aware Online Merge Planning with Learned Driver Behavior

Safe and reliable autonomy solutions are a critical component of next-generation intelligent transportation systems. Autonomous vehicles in such systems must reason about complex and dynamic driving scenes in real time and anticipate the behavior of nearby drivers. Human driving behavior is highly nuanced and specific to individual traffic participants. For example, drivers might display cooperative or non-cooperative behaviors in the presence of merging vehicles. These behaviors must be estimated and incorporated in the planning process for safe and efficient driving. In this work, we present a framework for estimating the cooperation level of drivers on a freeway and plan merging maneuvers with the drivers' latent behaviors explicitly modeled. The latent parameter estimation problem is solved using a particle filter to approximate the probability distribution over the cooperation level. A partially observable Markov decision process (POMDP) that includes the latent state estimate is solved online to extract a policy for a merging vehicle. We evaluate our method in a high-fidelity automotive simulator against methods that are agnostic to latent states or rely on $\textit{a priori}$ assumptions about actor behavior.

==> figs/hmm.tex <==
% https://texample.net/tikz/examples/kalman-filter/
\begin{figure}[t]

\centering

\tikzstyle{state}=[circle,
                                thick,
                                minimum size=1.2cm,
                                draw=vandeusen!80,
                                fill=vandeusen!20]

\tikzstyle{measurement}=[circle,
                                thick,
                                minimum size=1.2cm,
                                draw=cordovan!80,
                                fill=cordovan!25]

\begin{tikzpicture}[>=latex,text height=1.5ex,text depth=0.25ex]
    % "text height" and "text depth" are required to vertically
    % align the labels with and without indices.
  
  % The various elements are conveniently placed using a matrix:
  \matrix[row sep=0.5cm,column sep=0.5cm] {

        \\
        \node (A_k-2)         {$\cdots$};           &
        \node (x_k-1) [state] {$\mathbf{\theta}^{t-1}$}; &
        \node (x_k)   [state] {$\mathbf{\theta}^{t}$};     &
        \node (x_k+1) [state] {$\mathbf{\theta}^{t+1}$}; &
        \node (A_k+1)         {$\cdots$};     &      
        \\
        &
        \node (z_k-1) [measurement] {$\mathbf{y}^{t-1}$}; &
        \node (z_k)   [measurement] {$\mathbf{y}^{t}$};     &
        \node (z_k+1) [measurement] {$\mathbf{y}^{t+1}$}; &
        \\
        \\
    };
    
    % Connect the diagram elements with vectors
    \path[->]
        (A_k-2) edge[thick] (x_k-1)
        (x_k-1) edge[thick] (x_k)
        (x_k)   edge[thick] (x_k+1)
        (x_k+1) edge[thick] (A_k+1)
        
        (x_k-1) edge (z_k-1)
        (x_k)   edge (z_k)
        (x_k+1) edge (z_k+1)
        ;

\end{tikzpicture}

\caption{Hidden Markov model presenting the driver modeling task as a state estimation problem, as adapted from \citet{bhattacharyya2021hybrid}. $\theta^t$ are the latent cooperation level $c_T$ of the driver model and $\mathbf{y}^t$ are the observations from demonstration driving data. %The objective is to learn a distribution over the latent parameters from real-time observations using a recursive Bayesian filter.
}
\label{fig:hmm}
\end{figure}

==> related_work.tex <==
\section{Related Work}

The Intelligent Driver Model (IDM), developed by \citet{treiber2000congested}, is a rule-based adaptive cruise control model. The IDM is collision-free by construction and used for longitudinal motion modeling. It has inspired numerous extensions to capture microscopic driver behaviors. The Enhanced IDM prevents excessive breaking reactions due to lane changes, resulting in more relaxed and natural driving behavior \cite{kesting2010enhanced}. The Foresighted Driver Model is a risk-aware driver model that considers hazards such as obstacles and roadway curves \cite{eggert2015foresighted}. The Stochastic IDM attempts to model the stochasticity of human drivers by randomly sampling an output acceleration from a Gaussian distribution \cite{treiber2017intelligent}. In this work, we are concerned with freeway merge scenarios and thus consider the Cooperative Intelligent Driver Model proposed by \citet{bouton2019cooperation}. The C-IDM uses a simple deterministic model to represent the behavior of vehicles on the main lane in the presence of a merging vehicle. Both the The C-IDM and its foundational IDM framework are presented in more detail in the next section.

Rule-based driver models are governed by a relatively small number of parameters, which can be estimated in either an \textit{offline} or an \textit{online} fashion. Offline methods typically aggregate driving trajectory data in the training dataset and thus lose information on individual traffic participants. However, such methods can use arbitrarily large computation times and dataset sizes to maximize accuracy. Conversely, online methods must operate with constraints on computation time and data availability but capture the behavior of individual drivers. Offline strategies for rule-based driver model parameter estimation include constrained nonlinear optimization \cite{lefevre2014comparison}, the Levenberg-Marquardt algorithm \cite{morton2016analysis}, and genetic algorithms \cite{kesting2008calibrating}. Online strategies include Bayesian changepoint detection \cite{galceran2017multipolicy} and recursive Bayesian filters such as the Extended Kalman filter \cite{monteil2015real} and the particle filter \cite{bhattacharyya2021hybrid, buyer2019interaction, schulz2018interaction}. We employ a particle filter to conduct latent parameter estimation due to its ability to represent complex belief states.

Several papers have investigated interaction-aware planning for merge scenarios. \citet{ward2017probabilistic} consider merging on freeways and T-junctions; they fit parameters to an extension of the IDM using a nonlinear least-squares procedure. \citet{bouton2019cooperation} and \citet{ma2021reinforcement} conduct reinforcement learning-based techniques to learn merging policies. These works represent offline strategies for parameter estimation; we instead pursue an online strategy to capture the idiosyncrasies of individual drivers in real-time. The online parameter strategy presented by \citet{sunberg2020improving} is most similar to our approach; however, they only consider merging in lane change scenarios. We investigate freeway merging, which has been qualitatively described as one of the riskiest and complex driving maneuvers frequently encountered in day-to-day driving \cite{ward2017probabilistic}.


